Layout-induced Video Representation for Recognizing Agent-in-Place Actions

We address the recognition of agent-in-place actions, which are associated with agents who perform them and places where they occur, in the context of outdoor home surveillance. We introduce a representation of the geometry and topology of scene layouts so that a network can generalize from the layouts observed in the training set to unseen layouts in the test set. This Layout-Induced Video Representation (LIVR) abstracts away low-level appearance variance and encodes geometric and topological relationships of places in a specific scene layout. LIVR partitions the semantic features of a video clip into different places to force the network to learn place-based feature descriptions; to predict the confidence of each action, LIVR aggregates features from the place associated with an action and its adjacent places on the scene layout. We introduce the Agent-in-Place Action dataset to show that our method allows neural network models to generalize significantly better to unseen scenes.

==> backup.tex <==
\label{table:performance}
\scriptsize
% \ssmall
\begin{tabular}{@{}c|ccc|cccc|ccc|cc@{}}
\toprule
Network Architecture & \begin{tabular}[c]{@{}c@{}}B/L1\end{tabular} & \begin{tabular}[c]{@{}c@{}}B/L2\end{tabular} & \begin{tabular}[c]{@{}c@{}}B/L2 \\+MF\end{tabular}& \begin{tabular}[c]{@{}c@{}}Ours-\\V1\end{tabular}        & \begin{tabular}[c]{@{}c@{}}Ours-\\V2\end{tabular} &  \begin{tabular}[c]{@{}c@{}}Ours-\\V3\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}Ours-\\V4\end{tabular} & \begin{tabular}[c]{@{}c@{}}Ours-\\V4+H\end{tabular} & \begin{tabular}[c]{@{}c@{}}Ours-\\V4+MF\end{tabular} &
\begin{tabular}[c]{@{}c@{}}Ours-\\V4+FPS2\end{tabular} &
\begin{tabular}[c]{@{}c@{}}TSN \\\cite{tsn}\end{tabular} &
\begin{tabular}[c]{@{}c@{}}ReMotENet \\\cite{remotenet}\end{tabular}\\

\toprule
3D ConvNet?         & \checkmark                                                                                        & \checkmark                                                                                                       & \checkmark                                         & \checkmark                                             & \checkmark                                             & \checkmark                                                 & \checkmark                                                                 & \checkmark               &\checkmark                                                    &\checkmark  &-&-\\
ConcateMap?          &                                                                                                                  & \checkmark          &\checkmark                                                                                                       &                                                    &                                                        &                                                        &                                                            &                                                                            &                                                                             &&- &- \\
place-based feature description?                                                               &                                                              &           &                                                                                                       & \checkmark                                         & \checkmark                                             & \checkmark                                             & \checkmark                                                 & \checkmark                                                                 & \checkmark                                                                  &\checkmark   &- &- \\
distance-based place discretization?                                                               &                                                              &        &                                                                    &                                &                                             & \checkmark                                                 & \checkmark                                                                 & \checkmark                                                                & \checkmark  &\checkmark    &- &- \\
topological feature aggregation?                                                                  &                                                              &      &                                                                      &            & \checkmark                                                                                  &                                                        & \checkmark                                                 & \checkmark                                                                 & \checkmark                                                                 &\checkmark    &- &- \\
higher resolutions?                                        &                       &                                                              &                                                                                                                      &                                                    &                                                        &                                                        &                                                            & \checkmark                                                                 &                                                                             & & -&- \\
more filters?                                                               &                                                              &             & \checkmark                                                                                                                   &                                                    &                                                        &                                                        &                                                            &                                                                            & \checkmark                                                                  &  &- &- \\
higher FPS?                                   &                           &                                                              &                                                                                                                                &                                                    &                                                        &                                                        &                                                            &                                                                            &                                                                & \checkmark   &- &- \\
\midrule
Observed scenes mAP      & 43.34                                                               & 53.54           &        52.02                                      & 60.17      & \textbf{60.97}                                                                                          & 57.64                                                & 56.71                                                    & 56.26                                                         & 56.01                                                       & 58.93  &57.41 & 53.17\\
Unseen scenes mAP & 14.62                                                               & 20.96                &     16.12                                    & 41.54      & 44.73                                                                                          & 46.57                                                & 51.41                                                    & 49.13                                                         & \textbf{51.87}           &      50.31                                       
 &23.26 &21.13 \\ \bottomrule                                                   
\end{tabular}
\end{table*}
